Mono-Higgs and Mono-$Z$ Production in the Minimal Vector Dark Matter Model

The Minimal Vector Dark Matter is a viable realization of the minimal dark matter paradigm. It extends the Standard Model by the inclusion of a vector matter field in the adjoint representation of $SU (2)_L$. The dark matter candidate corresponds to the neutral component of the new vector field ($V^0$). Previous studies have shown that the model can explain the observed dark matter abundance while evading direct and indirect searches. At colliders, the attention has been put on the production of the charged companions of the dark matter candidate. In this work, we focus on the mono-Higgs and mono-$Z$ signals at hadron colliders. The new charged vectors ($V^{\pm}$) are invisible unless a dedicated search is performed. Consequently, we assume that the mono-Higgs and mono-$Z$ processes correspond the $pp\rightarrow h V^{+,0} V^{-,0}$ and $pp\rightarrow Z V^{+,0} V^{-,0}$ reactions, respectively. We show that, while the $p p \rightarrow h V^{+,0} V^{-,0}$ is more important, both channels may produce significant signals at the HL-LHC and colliders running at $\sqrt{s} = 27$ TeV and $100$ TeV, probing almost the complete parameter space.

==> respaldo.tex <==
\

\begin{thebibliography}{1}
  \bibitem{Cirelli:2005uq}Marco Cirelli, Nicolao Fornengo, and  Alessandro
  Strumia. {\newblock}Minimal dark matter. {\newblock}\tmtextit{Nucl. Phys.
  B}, 753:178--194, 2006.{\newblock}
  
  \bibitem{Saez:2018off}Bastian~D$\acute{\text{{\i}}}$az S{\'a}ez, Felipe
  Rojas-Abatte, and  Alfonso~R.~Zerwekh. {\newblock}Dark Matter from a Vector
  Field in the Fundamental Representation of $SU (2)_L$.
  {\newblock}\tmtextit{Phys. Rev. D}, 99(7):75026, 2019.{\newblock}
  
  \bibitem{Belyaev:2018xpf}Alexander Belyaev, Giacomo Cacciapaglia, James
  Mckay, Dixon Marin, and  Alfonso~R.~Zerwekh. {\newblock}Minimal Spin-one
  Isotriplet Dark Matter. {\newblock}\tmtextit{Phys. Rev. D}, 99(11):115003,
  2019.{\newblock}
  
  \bibitem{Abe:2020mph}Tomohiro Abe, Motoko Fujiwara, Junji Hisano, and 
  Kohei Matsushita. {\newblock}A model of electroweakly interacting
  non-abelian vector dark matter. {\newblock}\tmtextit{JHEP}, 07:136,
  2020.{\newblock}
  
  \bibitem{Zerwekh:2012bf}Alfonso~R.~Zerwekh. {\newblock}On the Quantum
  Chromodynamics of a Massive Vector Field in the Adjoint Representation.
  {\newblock}\tmtextit{Int. J. Mod. Phys. A}, 28:1350054, 2013.{\newblock}
  
  \bibitem{Belyaev:2020wok}Alexander Belyaev, Stefan Prestel, Felipe
  Rojas-Abbate, and  Jose Zurita. {\newblock}Probing dark matter with
  disappearing tracks at the LHC. {\newblock}\tmtextit{Phys. Rev. D},
  103(9):95006, 2021.{\newblock}

  %\cite{Belyaev:2012qa}
\bibitem{Belyaev:2012qa}
 A.~Belyaev, N.~D.~Christensen and A.~Pukhov,``CalcHEP 3.4 for collider physics within and beyond the Standard Model,''
 Comput. Phys. Commun. \textbf{184}, 1729-1769 (2013) doi:10.1016/j.cpc.2013.01.014{\newblock}


  \bibitem{ATLAS:2020fcp} G.~Aad \textit{et al.} [ATLAS], ``Measurements of $WH$ and $ZH$ production in the $H \rightarrow b\bar{b}$ decay channel in $pp$ collisions at 13 TeV with the ATLAS detector,''Eur. Phys. J. C \textbf{81}, no.2, 178 (2021).{\newblock}

  \bibitem{hepmdb}
M. Bondarenko, A. Belyaev, J. Blandford, L. Basso, E. Boos, V. Bunichev {\it et al.},
``High Energy Physics Model Database : Towards
decoding of the underlying theory" (within ``Les Houches 2011: Physics
at TeV Colliders New Physics Working Group Report"), arXiv:1203.1488
[hep-ph],
{https://hepmdb.soton.ac.uk}{\newblock}


  \bibitem{ATLAS:2021qou} G.~Aad \textit{et al.} [ATLAS], ``Measurement of Higgs boson decay into $b$-quarks in associated production with a top-quark pair in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector,''JHEP \textbf{06}, 097 (2022).{\newblock}

\bibitem{ATLAS:2022vkf}
 [ATLAS],``A detailed map of Higgs boson interactions by the ATLAS experiment ten years after the discovery,'' Nature \textbf{607}, no.7917, 52-59 (2022)[erratum: Nature \textbf{612}, no.7941, E24 (2022)].{\newblock} 
  

 \bibitem{Cepeda:2019klc} M.~Cepeda, S.~Gori, P.~Ilten, M.~Kado, F.~Riva, R.~Abdul Khalek, A.~Aboubrahim, J.~Alimena, S.~Alioli and A.~Alves, \textit{et al.}``Report from Working Group 2: Higgs Physics at the HL-LHC and HE-LHC,'' CERN Yellow Rep. Monogr. \textbf{7}, 221-584 (2019).{\newblock}
 
 \bibitem{FCC:2018vvp} A.~Abada \textit{et al.} [FCC],``FCC-hh: The Hadron Collider: Future Circular Collider Conceptual Design Report Volume 3,''
Eur. Phys. J. ST \textbf{228}, no.4, 755-1107 (2019).{\newblock}
 

\end{thebibliography}

\
